Convex Relaxations for Pose Graph Optimization with Outliers

Pose Graph Optimization involves the estimation of a set of poses from pairwise measurements and provides a formalization for many problems arising in mobile robotics and geometric computer vision. In this paper, we consider the case in which a subset of the measurements fed to pose graph optimization is spurious. Our first contribution is to develop robust estimators that can cope with heavy-tailed measurement noise, hence increasing robustness to the presence of outliers. Since the resulting estimators require solving nonconvex optimization problems, we further develop convex relaxations that approximately solve those problems via semidefinite programming. We then provide conditions under which the proposed relaxations are exact. Contrarily to existing approaches, our convex relaxations do not rely on the availability of an initial guess for the unknown poses, hence they are more suitable for setups in which such guess is not available (e.g., multi-robot localization, recovery after localization failure). We tested the proposed techniques in extensive simulations, and we show that some of the proposed relaxations are indeed tight (i.e., they solve the original nonconvex problem 10 exactly) and ensure accurate estimation in the face of a large number of outliers.

==> IRLSweightTable.tex <==
\begin{table}
{\renewcommand{\arraystretch}{2}
\cblue{
\begin{tabular}[h]{cc}
\hline
\hline
LOSS FUNCTION $\rho(\mathbf{r}_{i})$ & WEIGHTS $\mathbf{w}(\mathbf{r}_{i})$ \\ \hline
$\|\mathbf{r}_{i}\|_1$ & 
$\left[\frac{1}{|r_{i1}|}, \:\: \frac{1}{|r_{i2}|}\right]^{\top}$ \\ 
$\|\mathbf{r}_i\|_2$ & 
$\left[\frac{1}{\|\mathbf{r}_i\|_2}, \:\: \frac{1}{\|\mathbf{r}_i\|_2} \right]^{\top}$ \\ 
%$
%\begin{cases}
%\|x\|_2^2 \quad \text{if} \:\: |x|\leq 1 \\
%2 \|x\|_2 - 1 \quad \text{otherwise}
%\end{cases}
$\huber(\|\mathbf{r}_{i}\|_2)
$ & $[1, \:\: 1]^{\top} \cdot \begin{cases}
1 \quad \text{if} \:\: \|\mathbf{r}_{i}\|_2 \leq M \\
\frac{M}{\|\mathbf{r}_{i}\|_2} \quad \text{otherwise}
\end{cases} $\\ 
\hline
\hline
\end{tabular}
}}
\caption{\cblue{Weight functions associated to each robust cost function considered.}}
\label{IRLSweightsTable}
\end{table}

==> experiment-reweighted.tex <==
%!TEX root = Special Issue COMPENG2016 - Draft.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Re-weighted pose graph optimization for error mitigation}
A further possibility we explored is the use outliers detection to perform some sort of a refinement step after the procedure described in the previous section, consisting in the resolution of a re-weighted version of the SDP in which the new weights, ${\hat \omega}_k^T$ and ${\hat \omega}_k^R$, associated to each measurement in order to reduce the influence of outlying measurements on the solution. Hence we compute the refined solution ${\hat \MX}$ and the corresponding residuals ${\hat \restr}$ and ${\hat \resrot}$ by minimizing the cost function
\begin{align}
\label{eq:rewProb}
f({\hat \restr}, {\hat \resrot}) =  \sum_{k=1}^m {\hat \omega}_k^T  {\hat x}_k +  {\hat \omega}_k^R  {\hat y}_k
%\quad \text{s. to:}&\quad \|[\mathbf{X}]^{Rt}_{ij} -[\mathbf{X}]^{Rt}_{ii} - \Delta_{ij}\|_1 \leq {\hat x}_k,\quad k=1,\dots,m \nonumber\\
%& \quad \|[\mathbf{X}]^{RR}_{ij} -\bar{ R}_{ij}\|_1 \leq {\hat y}_k,\quad k=1,\dots,m \nonumber\\
%&\quad [\mathbf{X}]^{RR}_{ii}=I_2,\quad i=1,\dots,n \nonumber\\
%& \quad \mathbf{X} \succeq 0  \nonumber
\end{align}

where
\begin{align}
\label{eq:newWeights}
{\hat \omega}_k^T = \frac{1}{\max\{\eta^T,\: x_k\}} \quad \text{and} \quad {\hat \omega}_k^R = \frac{1}{\max\{\eta^R,\: y_k\}}
\end{align}

Again, a suitable choice of the thresholds $\eta^T$ and $\eta^R$ could be respectively $2\sigma_T$ and $2\sigma_R$.

We tested the effectiveness of this ``refinement'' technique based on the solution yielded by the {\itshape $\ell_2$ 2-stage} formulation, since it is the most probabilistically grounded among the ones that showed the highest performance in detecting outliers (see Subsection~\ref{sec:OutIdentifResults}). In Fig.~\ref{fig:rewImprovement} is reported the mean error over each position and orientation before (blu line) and after the re-weighted optimization (red line). We observe a reduction of the mean rotation and translation error for all values of $p^{out}$ and on both tests with $20$ and $50$ nodes. Although the rotation error decrease is very small, the mean translation error drops by around $5$cm in just 1 run of re-weighted optimization. However, this improvement becomes smaller for larger instances, which is consistent with what we observe in Fig.~\ref{fig:aveDistFromGTn}. 
In conclusion, these results prove that through the introduction of the re-weighted cost function proposed in Eqs.~\eqref{eq:rewProb} and \eqref{eq:newWeights} we are actually able to mitigate the influence of outliers in the optimization, improving the pose estimate. 
\begin{figure}[h]
\begin{minipage}{\columnwidth}
\begin{tabular}{cc}
\hspace{-5 mm}
\begin{minipage}{0.5\columnwidth}%
\includegraphics[scale=0.22]{figures/REWtrann20}  \\ 
\end{minipage}%
&
\hspace{-3 mm}
\begin{minipage}{0.5\columnwidth}%
\centering
\vspace{-3.5mm}
\includegraphics[scale=0.22]{figures/REWrotn20}  \\ 
\end{minipage}%  
\end{tabular} \\
\centering
\end{minipage}%
\caption{Improvement of the estimated solution obtained through re-weighted optimization: mean rotation and translation errors associated to the solutions of the {\itshape $\ell_2$ 2-stage} formulation, with $\sigma_R = 0.01$, $\sigma_T = 0.1$, $p=0.5$ and $n=20$.
\label{fig:rewImprovement}}
\end{figure}


==> experiments-IRLS.tex <==
%!TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\cblue{Fast numerical solver}}
\label{sec:FastNumericalSolver}
\cblue{In this section we propose an approximation method that allows to solve the {\itshape 2-stage} approaches proposed in Section~\ref{sec:2stage} by leveraging the method of {\itshape Iteratively Reweighted Least Squares} (IRLS). The use of IRLS for robust linear regression is not new and in literature there exist extensive discussion of its \cred{statistical justification,} implementation and effectiveness~\cite{hollandwelsch} \cred{[others?]}.}

\cblue{
Firstly, we reformulate problems \eqref{eq:huberOnRot-relax}, and \eqref{eq:tranSubproblem} -- corresponding, respectively, to the rotation and translation PGO subproblems -- by introducing a different parametrization of rotation as vectors in $	\Real{2}$
\begin{equation}
\mathbf{r}_i = [ \text{cos}(\theta_i), \:\:\: \text{sin}(\theta_i)]^{\top} \quad \text{for} \:\: i=1,\dots,n 
\end{equation}
where $\theta_i$ is the rotation angle corresponding to $\MR_i$, formerly used.
%\begin{align}
%\mathbf{r}_i = \left[ \begin{array}{c} \text{cos}(\theta_i) \\ \text{sin}(\theta_i) \end{array} \right]
%\end{align}
This leads to the following optimization problems in $\mathbf{r} = [\mathbf{r}_1^{\top}, \dots, \mathbf{r}_n^{\top}]^{\top}\in \Real{2n}$ and $\mathbf{t}\in \Real{2n}$:
\begin{eqnarray}
\min_{\mathbf{r}} \:\:\:  & \sum_{k=1}^m \: \!\! f_R(\mathbf{\bar U}_k \mathbf{r}) \\
\subject & \|\mathbf{r}_i\|_2 = 1, \quad i = \,\dots, n \nonumber
\label{eq:IRLSstage1problem}
\end{eqnarray}
for the generic first stage, and 
\begin{align}
\min_{\mathbf{p}} \:\:\:  & \sum_{k=1}^m \: \!\! f_t(\mathbf{\bar A}_k \mathbf{p}+\mathbf{\bar D}_k \mathbf{r})
\label{eq:IRLSstage2problem}
\end{align}
for the second stage, where $\mathbf{\bar U}_k$, $\mathbf{\bar A}_k$ and $\mathbf{\bar D}_k$ are the generic $k$-th block row of matrices $\mathbf{\bar U} \in \Real{2m\times2n}$, $\mathbf{\bar A} \in \Real{2m\times2n}$ and $\mathbf{\bar D} \in \Real{2m\times2n}$ respectively, which are defined as per \cred{[Carlone16tro-duality2D]}.}
%\begin{align}
%\mathbf{\bar U} = \left[ \begin{array}{c} \mathbf{\bar U}_1 \\ \vdots \\ \mathbf{\bar U}_m \end{array} \right] \in \Real{2m\times2n}, \:\: \mathbf{\bar A} = \left[ \begin{array}{c} \mathbf{\bar A}_1 \\ \vdots \\ \mathbf{\bar A}_m \end{array} \right] \in \Real{2m\times2n} \:\: \text{and} \mathbf{\bar D} = \left[ \begin{array}{c} \mathbf{\bar D}_1 \\ \vdots \\ \mathbf{\bar D}_m \end{array} \right] \in \Real{2m\times2n}
%\end{align}}

\cblue{Then, we relaxate problem~\eqref{eq:IRLSstage1problem} by considering the unconstrained minimization of its cost function, from which we get a linear regression problem in variable $\mathbf{r}$. Note that problem~\eqref{eq:IRLSstage2problem} is already a linear regression problem in the variable $\mathbf{p}$, so both stages are now optimization problems that can be cast in the following general form of a linear regression problem}
\cblue{
\begin{align}
y = X \pmb{\beta} + \epsilon
\end{align}
where $\epsilon$ is the measurement noise and we aim at estimating the model parameter $\pmb{\beta}$ that best fit the data:
\begin{align}
\hat{\pmb{\beta}} =\arg \min_{\pmb{\beta}} \sum_{k=1}^m f(y_k - X_k \pmb{\beta}).
\end{align}}
\cblue{The IRLS method consists in an iterative routine in which at each step a {\itshape weighted least squares} problem in the form}
%\cblue{
%\begin{align}
%\hat{\pmb{\beta}}^{(k+1)} =\arg \min_{\pmb{\beta}} \sum_{i=1}^m \mathbf{w}_i(\pmb{\beta}^{(k)}) \cdot |y_i - X_i \pmb{\beta} |^2 
%\end{align}}
\cblue{
%or, in matrix form,
\begin{align}
\hat{\pmb{\beta}}^{(t+1)} = ( X^{\top} W^{(t)} X)^{-1} X^{\top}W^{(t)} y
\end{align}
is solved, where matrix $W^{(t)}\in \Real{2m\times2m}$ is updated at each step $t$ as function of the residuals $\mathbf{r}_k(\pmb{\beta}^{(t)}) = \mathbf{y}_{k} - X_k\pmb{\beta}$ for $k=1,\dots, m$, associated to the $m$ measurements:
 \begin{equation}
 %W^{(k)} = \diag{[\mathbf{w}_1(\pmb{\beta}^{(k)})^{\top}, \dots, \mathbf{w}_m(\pmb{\beta}^{(k)})^{\top}]^{\top}} 
 W^{(k)} = \diag{[\mathbf{w}(\mathbf{r}_1^{(k)})^{\top}, \dots, \mathbf{w}(\mathbf{r}_m^{(k)})^{\top}]^{\top}}.
 \end{equation}
The {\itshape weight function} $\mathbf{w}(\cdot)$ is suitably chosen in order to minimize the specific robust costs $f_R(\cdot)$ and $f_t(\cdot)$, as reported in Table~\ref{IRLSweightsTable} for the three loss functions considered in this work. While convergence has been proven for the $\ell_1$-norm and Huber loss \cite{chartrand2008iteratively}, \cite{hollandwelsch}, the choice of the weights for Least Unsquared Deviation reported in Table~\ref{IRLSweightsTable} has been taken by analogy with respect to the case in which we aim to minimize the $\ell_2$-norm of the whole vector of translation residuals and Frobenius norm of rotation residuals instead of the sum of the norms of each pose's residual. Although not having {\itshape a priori} guarantees of convergence for this choice, results show empirically that such weights actually fit our purpose.} 

\cblue{Fig.~\ref{fig:IRLSapproxPrecision} shows the average approximation error over translations obtained when IRLS is employed only to solve the translation subproblem based on the orientations estimate obtained by solving subproblem~\eqref{eq:huberOnRot-relax} (red line), versus the error when IRLS is used to solve both stages of the techniques under consideration (blue line) for increasing probability of outliers $p^{out}$. We use this metric as measure of the precision of the IRLS approximation since it also allows to evaluate the error accumulation over the two stages. The translation mismatch with respect to the solution of the corresponding convex relaxation solved via \cvx, is measured with $\ell_2$-norm, while the metric employed for average rotation mismatch is the absolute value of the modulo-$\pi$ difference of nodes headings. For $n=50$ and all graph model employed in this work, the average translation mismatch is always lower than $5 \:\text{cm}$, even for the highest levels of outliers considered. Precision increases with the number of nodes and the level of connectivity of the graph.}

\cred{To be explained:
\begin{itemize}
\item justification of the weights exists only for Huber (ref holland-welsch) and $\ell_1$ (check it)
\item why unconstrained minimization of robust cost works for getting feasible solutions via rounding procedures? Maybe Luca mentioned a ref once...
\item all IRLS techniques work well in practice(a posteriori guarantees of convergence)
\end{itemize}
}

\begin{figure*}[h]
\begin{minipage}{\textwidth}
\begin{tabular}{ccc}
\hspace{-5 mm}
\begin{minipage}{0.33\textwidth}%
\includegraphics[scale=0.3]{figures/gray}  \\ 
%\includegraphics[scale=0.3]{figures/IRLS-L1OverTran_Vs_IRLSooverBoth_Erd50}  \\ 
\centering (a)
\end{minipage}%
&
\hspace{-1.5 mm}
\begin{minipage}{0.33\textwidth}%
\centering
%\vspace{-3.5mm}
\includegraphics[scale=0.3]{figures/IRLS-L2OverTran_Vs_IRLSooverBoth_Erd50}  \\ 
\hspace{0 mm}
\centering (b)
\end{minipage}% 
&
\hspace{-1.5 mm}
\begin{minipage}{0.33\textwidth}%
\includegraphics[scale=0.3]{figures/gray}  \\ 
\includegraphics[scale=0.3]{figures/IRLS-HuberOverTran_Vs_IRLSooverBoth_Erd50}  \\ 
\centering (c)
\end{minipage} 
\end{tabular} 
\end{minipage}%
\caption{\cblue{Error of IRLS approximation for the three 2-stage approaches considered: (a) $\ell_1$ {\itshape 2-stage}, (b) $\ell_2$ {\itshape 2-stage} and (c) {\itshape Huber 2-stage}, all measured over tests with $n=50$ poses and edges generated according to {\itshape Erd\H os-R\'enyi} random graph model.}}
\label{fig:IRLSapproxPrecision}
\end{figure*}

\input{IRLSweightTable}


\begin{figure}[h]
\begin{minipage}{\columnwidth}
\begin{tabular}{cc}
\hspace{-5 mm}
\begin{minipage}{0.5\columnwidth}%
\includegraphics[scale=0.235]{figures/comparAveTran_Erdos100}  \\ 
\end{minipage}%
&
\hspace{-3 mm}
\begin{minipage}{0.5\columnwidth}%
\centering
\vspace{-3.5mm}
\includegraphics[scale=0.235]{figures/comparAveRot_Erdos100}  \\ 
\end{minipage}%  
\end{tabular} \\
\centering
(a) {\footnotesize  \cblue{{\itshape Erd\H os-R\'enyi}, $n=100$.}}
\end{minipage}%
\\
\begin{minipage}{\columnwidth}
\begin{tabular}{cc}
\hspace{-5 mm}
\begin{minipage}{0.5\columnwidth}%
\includegraphics[scale=0.235]{figures/comparAveTran_Erdos200}  \\ 
\end{minipage}%
&
\hspace{-3 mm}
\begin{minipage}{0.5\columnwidth}%
\centering
\vspace{-3.5mm}
\includegraphics[scale=0.235]{figures/comparAveRot_Erdos200}  \\ 
\end{minipage}%
\end{tabular}\\
\centering
(b) {\footnotesize  \cblue{{\itshape Erd\H os-R\'enyi}, $n=200$.}} % $\sigma_R = 0.01$, $\sigma_T = 0.1$, $p=0.5$,
\end{minipage}%
\\
\begin{minipage}{\columnwidth}
\begin{tabular}{cc}
\hspace{-5 mm}
\begin{minipage}{0.5\columnwidth}%
\includegraphics[scale=0.235]{figures/comparAveTran_Geo100}  \\ 
\end{minipage}%
&
\hspace{-3 mm}
\begin{minipage}{0.5\columnwidth}%
\centering
\vspace{-3.5mm}
\includegraphics[scale=0.235]{figures/comparAveRot_Geo100}  \\ 
\end{minipage}%  
\end{tabular} \\
\centering
(c) {\footnotesize \cblue{{\itshape Geometric}, $n=100$.}}
\end{minipage}%
\\
\begin{minipage}{\columnwidth}
\begin{tabular}{cc}
\hspace{-5 mm}
\begin{minipage}{0.5\columnwidth}%
\includegraphics[scale=0.235]{figures/comparAveTran_Geo200}  \\ 
\end{minipage}%
&
\hspace{-3 mm}
\begin{minipage}{0.5\columnwidth}%
\centering
\vspace{-3.5mm}
\includegraphics[scale=0.235]{figures/comparAveRot_Geo200}  \\ 
\end{minipage}%  
\end{tabular} \\
\centering
(d) {\footnotesize\cblue{{\itshape Geometric}, $n=200$.}}
\end{minipage}%
\cblue{\caption{Estimation errors for the {\itshape 2-stage} approaches solved via IRLS compared with state-of-the-art techniques: g2o and DCS.
Left column: average translation error. Right column: average rotation error. 
 {\itshape Erd\H os-R\'enyi} random graphs with (a) $n=100$ and (b) $n=200$ nodes; {\itshape Geometric} random graphs with (c) $n=100$ and (d) $n=200$ nodes.}
%Errors are computed with respect to the ground truth.
% Comparison of the quality of the estimated pose configuration provided by the different approaches, in terms of mean estimation error over the single position and orientation of a node.
\label{fig:aveDistFromGT_big}}
\end{figure}

==> experiments-poseGraphExample.tex <==
%!TEX root = main.tex

\red{
 In Fig.~\ref{fig:graphs}  we provide an example of pose configuration estimates obtained with {\itshape 1-} and {\itshape 2-stage} approaches based on the same norm (in this case, {\itshape unsquared} $\ell_2$), compared with the ground truth configuration (poses in grey). Outliers are highlighted as red dotted lines. The solution yielded by the 2-stage approach is visibly more accurate that the one obtained with the corresponding 1-stage approach, and overlaps almost perfectly  with the ground truth poses. 
}
  \begin{figure}[h]
\begin{minipage}{\columnwidth}
\begin{tabular}{cc}
\hspace{-5 mm}
\begin{minipage}{0.5\columnwidth}%
\includegraphics[scale=0.38]{figures/graphWangOnPoses-01}  \\ 
\centering (a) 
\end{minipage}%
&
\hspace{ -3mm}
\begin{minipage}{0.5\columnwidth}%
\centering
%\vspace{-3.5mm}
\includegraphics[scale=0.38]{figures/graphWang2stage-01}  \\ 
\centering (b) 
\end{minipage}%  
\end{tabular} 
\end{minipage}%
\red{\caption{Example of estimated poses via (a) {\itshape $\ell_2$ on poses} and 
(b) {\itshape $\ell_2$ 2-stage} approaches, compared with the ground truth configuration (grey).} 
%$\sigma_R = 0.01$, $\sigma_T = 0.1$, $p=0.5$, $p^{out}=0.2$ and $n=20$.
\label{fig:graphs} }
\end{figure}


==> experiments-relaxGap.tex <==
%!TEX root = main.tex

The effectiveness of the convex relaxation in the
%The tightness of the 
2-stage approaches is confirmed by the behavior of the relative rounding gap, i.e. the relative difference between the cost of the rounded solution and the optimal cost of the SDP relaxation.
% and the cost of the rounded solution
%associated to the feasible solution obtained through rotation rounding. 
Fig.~\ref{fig:RGAP} shows that all 2-stage techniques have a very small rounding gap 
for all values of $p^{out}$, while 1-stage techniques have large rounding gaps (above $50\%$). Note that in absence of outliers ($p^{out}=0$) the relative rounding gap is higher than in presence of outliers ($p^{out}\geq0.05$). 
This is mainly due to the fact that the presence of outliers significantly increases the costs associated to both the solution of the SDP relaxation and the rounded solution, making the relative rounding gap smaller.
%while the increase of the rounding gap is less than proportional.   
%This figure further confirms that the convex relaxation in the 2-stage approaches 
% produces accurate solutions to the original (decoupled) problem.

\begin{figure}[h]
\begin{minipage}{\columnwidth}
\begin{tabular}{cc}
\hspace{-5 mm}
\begin{minipage}{0.5\columnwidth}%
\includegraphics[scale=0.235]{figures/RGAPn20sigmaR001}  \\ 
\centering (a) $n=20$
\end{minipage}%
&
\hspace{-3 mm}
\begin{minipage}{0.5\columnwidth}%
\centering
%\vspace{-3.5mm}
\includegraphics[scale=0.235]{figures/RGAPn50sigmaR001}  \\ 
\centering (b) $n=50$
\end{minipage}%  
\end{tabular} 
\end{minipage}%
\caption{Rounding gap for increasing probability of outliers with
 (a)  $n=20$ (b) $n=50$ unknown poses.
\label{fig:RGAP}}
\end{figure}

==> experiments-residuals.tex <==
%!TEX root = main.tex

Fig.~\ref{fig:outDetExample}(a) shows the translation residuals (solid blue line)
while Fig.~\ref{fig:outDetExample}(b) shows the rotation residuals (solid red line)
for a test instance with $n=50$ poses. Triangles denote the outliers generated as per \eqref{eq:modelOutTran}; 
red triangles label rotation-only outliers, 
blue triangles denote translation-only outliers, and green one denote outliers on the full pose measurement. 
From Fig.~\ref{fig:outDetExample}(a) we see that the outliers on translations and on the full poses 
clearly correspond to larger translation residuals, and can be easily identified, imposing a 
suitable threshold, e.g., $\eta^t = 1\meter$. 
Similarly, from Fig.~\ref{fig:outDetExample}(b) we see that the outliers on rotations and on the full poses 
clearly correspond to larger rotation residuals.
% Very often, peaks correspond to outliers and by fixing suitable thresholds (dashed lines in Fig.~\ref{fig:outDetExample}), one can efficiently classify measurements as inliers (peaks below the threshold) or outliers (peaks above the threshold). 

\begin{figure}[h]
\begin{minipage}{\columnwidth}
\begin{tabular}{cc}
\hspace{-5 mm}
\begin{minipage}{0.5\columnwidth}%
\includegraphics[scale=0.235]{figures/OutDetectTran_n50sigmaR001} 
\end{minipage}%
&
\hspace{-3 mm}
\begin{minipage}{0.5\columnwidth}%
\centering
%\vspace{-3.5mm}
\includegraphics[scale=0.235]{figures/OutDetectRot_n50sigmaR001}  
\end{minipage}%  
\end{tabular} 
\end{minipage}%
\caption{Example of outliers detection procedure on an instance with 
%$\sigma_R = 0.01$, $\sigma_T = 0.1$, $p=0.5$, 
$n=50$ poses. Blue triangles are translation-only outliers, red ones are rotation-only outliers,
 and green ones are to outliers on both rotations and translations. The dashed lines represent a possible 
 choice of the thresholds $\eta^t$ and $\eta^R$, which separate inliers (below threshold) form outliers (above threshold).
\label{fig:outDetExample} }
\end{figure}

==> figureResults1.tex <==
%!TEX root = main.tex

\begin{figure}[h]
\begin{minipage}{\columnwidth}
\begin{tabular}{ccc}
\rotatebox{90}{{\footnotesize \hspace{-1cm}{(a) \itshape Erd\H os-R\'enyi}, $n=20$}}
&
\hspace{-5 mm}
\begin{minipage}{0.45\columnwidth}%
\includegraphics[scale=0.235]{figures/comparAveTran_Erdos20}  \\ 
\end{minipage}%
&
\hspace{-3 mm}
\begin{minipage}{0.45\columnwidth}%
\centering
\vspace{-3.5mm}
\includegraphics[scale=0.235]{figures/comparAveRot_Erdos20}  \\ 
\end{minipage}%  
\end{tabular} 
% \\
% \centering
% (a) {\footnotesize  {\itshape Erd\H os-R\'enyi}, $n=20$.}
\end{minipage}%
\\
\begin{minipage}{\columnwidth}
\begin{tabular}{ccc}
\hspace{-5 mm}
\begin{minipage}{0.5\columnwidth}%
\includegraphics[scale=0.235]{figures/comparAveTran_Erdos50}  \\ 
\end{minipage}%
&
\hspace{-3 mm}
\begin{minipage}{0.5\columnwidth}%
\centering
\vspace{-3.5mm}
\includegraphics[scale=0.235]{figures/comparAveRot_Erdos50}  \\ 
\end{minipage}%
\end{tabular}\\
\centering
(b) {\footnotesize  {\itshape Erd\H os-R\'enyi}, $n=50$.} % $\sigma_R = 0.01$, $\sigma_T = 0.1$, $p=0.5$,
\end{minipage}%
\\
\begin{minipage}{\columnwidth}
\begin{tabular}{ccc}
\hspace{-5 mm}
\begin{minipage}{0.5\columnwidth}%
\includegraphics[scale=0.235]{figures/comparAveTran_Geo20}  \\ 
\end{minipage}%
&
\hspace{-3 mm}
\begin{minipage}{0.5\columnwidth}%
\centering
\vspace{-3.5mm}
\includegraphics[scale=0.235]{figures/comparAveRot_Geo20}  \\ 
\end{minipage}%  
\end{tabular} \\
\centering
(c) {\footnotesize {\itshape Geometric}, $n=20$.}
\end{minipage}%
\\
\begin{minipage}{\columnwidth}
\begin{tabular}{ccc}
\hspace{-5 mm}
\begin{minipage}{0.5\columnwidth}%
\includegraphics[scale=0.235]{figures/comparAveTran_Geo50}  \\ 
\end{minipage}%
&
\hspace{-3 mm}
\begin{minipage}{0.5\columnwidth}%
\centering
\vspace{-3.5mm}
\includegraphics[scale=0.235]{figures/comparAveRot_Geo50}  \\ 
\end{minipage}%  
\end{tabular} \\
\centering
(d) {\footnotesize {\itshape Geometric}, $n=50$.}
\end{minipage}%
\caption{Estimation errors for the 6 approaches proposed in this paper.
Left column: average translation error. Right column: average rotation error. 
 {\itshape Erd\H os-R\'enyi} random graphs with (a) $n=20$ and (b) $n=50$ nodes; {\itshape Geometric} random graphs with (c) $n=20$ and (d) $n=50$ nodes.
%Errors are computed with respect to the ground truth.
% Comparison of the quality of the estimated pose configuration provided by the different approaches, in terms of mean estimation error over the single position and orientation of a node.
\label{fig:aveDistFromGT_small}}
\end{figure}

==> multirobotLocalization.tex <==
%!TEX root = Special Issue COMPENG2016 - Draft.tex

\section{\cblue{Multi-robot Localization from Relative Pose Measurements}}
\label{sec:PGO}
%
\cblue{The problem of multi-robot localization consists of estimating the poses of the $n$ robots from $m$ noisy measurements of relative poses between them.
Assuming each robot to be denoted by a unique identification number $i \in \{1,\dots,n\}$, in the planar setup} each to-be-estimated pose $\vxx_i \doteq (\MR_i,\vt_i)$, $i=1,\ldots,n$,
 comprises a \emph{translation} vector $\vt_i \in \Real{2}$  
and a rotation matrix $\MR_i \in \SOtwo$ \cblue{encoding position and orientation of robot $i$, respectively}.
For a pair of poses $(i,j)$, 
a relative pose measurement $\barx\ij \doteq (\barR\ij,\bart\ij)$, with $\bart\ij \in \Real{2}$ and 
$\barR\ij \in \SOtwo$,
 describes a noisy measurement of 
the relative \cblue{position and orientation between robot $i$ and $j$.} %the two unknown poses.
Each measurement is assumed to be sampled from the following
\emph{generative  model}:
\begin{align}
\label{eq:noisyModel}
\bart\ij = \MR_i\tran (\vt_j - \vt_i ) + \noiset\ij, \quad \quad \barR_{ij} = \MR_i\tran \MR_j \noiseR_{ij}
\end{align}
where $\noiset\ij \in \Real{2}$ 
and $\noiseR_{ij} \in \SOtwo$ represent translation and rotation measurement noise, respectively.
% The generic $k$-th edge, connecting the nodes $i$ and $j$, is labeled with the pair $(\Delta_{ij}, R_{ij})$ containing respectively the relative position and rotation of $j$ with respect to $i$. In a noiseless setup, these quantities verify the following relations:
% \begin{align}
% \label{eq:noiselessModel}
% \Delta_{ij} = R_i^{\top} (t_j - t_i ), \quad \quad R_{ij} = R_i^{\top}R_j.
% \end{align}

The problem can be elegantly modeled through \cblue{a directed graph ${\calG}({\calV},{\calE})$, where}
each to-be-estimated pose is a associated to a vertex (or node) in the vertex set ${\calV}$, while each given measurement is associated to an edge in 
the edge set $\calE$ of the graph. We denote by $n\doteq |\calV|$  the number of nodes
and by $m\doteq |\calE|$  the number of edges.

\subsection{Standard \cblue{formulation}}
\label{sec:standardPGO}

Given the generative model~\eqref{eq:noisyModel}, standard approaches to \cblue{multi-robot localization} 
formulate the pose estimation problem in terms of \emph{maximum likelihood} (ML) estimation: 
the best pose estimate is the one maximizing the likelihood of the available measurements
 $\barx\ij, \forall (i,j) \in \calE$.

 The first step to design a maximum likelihood estimator is to assume suitable distributions for the 
 measurement noise. An ubiquitous assumption is that the translation noise $\noiset\ij$ 
 is distributed according to a zero-mean Normal distribution with given covariance $\MSigma^t\ij$, 
 i.e., $\noiset\ij \sim \gaussian(\zero,\MSigma^t\ij)$. 
% nodes in ${\mathcal V}$ are labelled with the poses assumed by the robot in different instants of time, while the set of the edges ${\mathcal E}$ represents the set of pairwise spacial constraints extracted from the raw measurements acquired by the robot during operation. In this paper, the graph ${\mathcal G}$ underlying the PGO problem is assumed to be always connected.
% Accordingly, the generic $i$-th node is labeled with the $i$-th pose $x_i = (t_i, R_i)$, where the vector $t_i \in \Real{2}$ is the position in the plane and $R_i \in \text{SO}(2)$ is the orientation of the robot parametrized by a rotation matrix. 
% In this condition, the PGO problem reduces to a system of linear equations in the unknowns $\{t_i\}_{i=1}^n$ and  $\{R_i\}_{i=1}^n$ that, assuming the underlying graph connected, admits a unique solution up to a global roto-translation.
% \subsection{Noise assumptions}
% \label{sec:noiselessAssumptions}
% In presence of noise, the relations~\eqref{eq:noiselessModel} become:
% Outlying (incorrect) translation and rotation measurements are assumed to be generated by adding an additive disturbance $({\tilde \Delta}_{ij}, {\tilde R}_{ij})$ to the relative pose, distributed according to a uniform (Haar) distribution \cred{over} respectively $\Real{2}$ and $\text{SO}(2)$, which yields the following relations:
% \begin{align}
% \label{eq:outlierModel}
% \Delta_{ij} = R_i^{\top} (t_j - t_i ) + {\tilde \Delta}_{ij}, \quad \quad R_{ij} = R_i^{\top}R_j+ {\tilde R}_{ij}.
% \end{align}
% This assumption is also used in \cred{[Wang]}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Pose Graph Optimization}
% \cblue{In general, when measurements are noisy, there is no estimate that satisfies exactly~\eqref{eq:noiselessModel} for all measurements $(i,j) \in {\mathcal E}$. Therefore, one rather looks for a set of positions $\{t_1, \dots, t_n\}$ and rotations $\{R_1 , \dots, R_n \}$ that minimizes the mismatch with respect to the measurements.} 
%In other words, we need to address a {\itshape maximum likelihood estimation} problem. 
For the rotation noise, a fairly popular assumption is that the rotation noise is 
distributed according to a wrapped Gaussian distribution; we refer the reader to~\cite{Carlone14tro} 
for a comprehensive discussion on the wrapped Gaussian and the corresponding maximum likelihood 
estimator. 
% \begin{align}
% \label{eq:wrappedGaussian}
% \noiseR\ij = \expmap{\theta_\epsilon}, \quad \quad \theta_\epsilon \sim \calN(0,\sigma^R\ij)
% \end{align}
More recently, it has been proposed to use the Von Mises distribution for the rotation noise, as 
this leads to simpler estimators and is easier to analyze~\cite{Carlone16tro-duality2D}.
In particular, it is assumed that the rotation noise $\noiseR\ij$ in~\eqref{eq:noisyModel} 
is a rotation of a random angle $\noiseTheta$ and this angle is distributed according 
to the Von Mises distribution:
\begin{align}
\label{eq:wrappedGaussian}
\vonMises(\noiseTheta; \mu, \kappa) = 
c(\kappa) \exp(\kappa \cos(\noiseTheta - \mu) )
\end{align}
with mean $\mu$, concentration parameter $\kappa$, and 
where $c(\kappa)$ is a normalization constant whose expression is irrelevant for the
purpose of the estimation.
 % is distributed according to a zero-mean normal distribution with covariance $\frac{1}{\omega^{\Delta}}\cdot I_2$, while ${\tilde R}_{ij}$ is sampled from a \cred{Von Mises-Fischer} distribution centered in zero with concentration parameter $\omega^{R}$.

 These choices of the noise model lead to the following standard PGO formulation 
 (for simplicity we restrict ourselves to the case of isotropic noise, i.e., 
 the matrix $\MSigma^t\ij$ is assumed to be diagonal).

 \begin{proposition}[Standard PGO formulation]
 \label{prop:standardPGO}\ \\
 Given the generative model~\eqref{eq:noisyModel} and assuming that the 
 translation noise is $\noiset\ij \sim \emph{\gaussian}(\zero, \frac{1}{\omegat\ij} \eye_2)$  
 and the rotation noise is $\noiseR\ij \sim \emph{\vonMises}(\zero, \omegaR\ij)$, then the 
 maximum likelihood estimate of the poses is the minimizer of the  optimization problem
 \begin{align}
\!\!\!\min_{\constraints}  \sumalledges \!\!
\omegat\ij \|\MR_{i}\tran(\vt_j\!-\!\vt_i)\!-\!\bart_{ij}\|^2_2 
\!+\! \frac{\omegaR_{ij}}{2} \|\MR_{i}\tran \!\MR_j \!-\!\barR_{ij}\|^2_F 
%\nonumber\\
\label{eq:Squaredl2OnPosesPrimal}
% \quad \subject&\quad R_i \in SO(2), \quad i=1,\dots,n 
\end{align}
 \end{proposition}
% Under the noise assumptions as per~\eqref{eq:noisyModel}, the maximum likelihood estimation corresponds to the solution of the following optimization problem \cred{[Ref TRO]}:
% which is {\itshape non-convex} due to non-convexity of its feasible set.
%
A proof of this statement is given  in~\cite[Proposition 1]{Carlone16tro-duality2D}.
The standard ML estimator~\eqref{eq:Squaredl2OnPosesPrimal} entails  a nonconvex optimization 
problem, due to the nonconvexity of the set $\SOtwo$.
Surprisingly, 
recent results~\cite{Carlone16tro-duality2D} show that 
one can still compute a globally optimal solution to~\eqref{eq:Squaredl2OnPosesPrimal} 
whenever the measurement noise is reasonable, practically covering 
the noise regimes commonly found in all robotics and computer vision applications.

The main issue with the formulation~\eqref{eq:Squaredl2OnPosesPrimal} is that 
it produces unreasonable results in presence of \emph{outliers}, i.e., measurements 
that do not follow the noise assumptions of Proposition~\ref{prop:standardPGO}, hence 
lacking robustness. % robust operation.

This work extends our previous work~\cite{Carlone16tro-duality2D} to consider  
more robust cost functions, which enable reliable estimation in the face of a large number of 
outliers. Similarly to~\cite{Carlone16tro-duality2D} these formulations lead to 
nonconvex problems and we resort to convex relaxations. 
However, contrarily to~\cite{Carlone16tro-duality2D} we propose a more systematic and 
direct way to design convex relaxations and we show that 
the performance of the relaxations are fundamentally different from the 
standard formulation in Proposition~\ref{prop:standardPGO}.
% uses Lagrangian duality as a tool to 
% obtain a convex relaxation of problem~\eqref{eq:Squaredl2OnPosesPrimal}. 
% In this work, we present a more direct approach to obtain convex relaxations and 
% we extend~\eqref{eq:Squaredl2OnPosesPrimal} to the use of   
% one can still compute a global 
% minimum of~\eqref{eq:Squaredl2OnPosesPrimal} by using Lagrangian duality. 
% The surprising finding of~\cite{Carlone16tro-duality2D} is that despite its nonconvexity, 
% problem~\eqref{eq:Squaredl2OnPosesPrimal} has a 
% This formulation, although allowing for the computation of a guaranteed globally optimal solution through convex relaxation even under very high levels of noise \cred{[Ref TRO]}, \cred{shows no robustness with respect to incorrect measurements.} This has driven our investigation towards the use of more  ``robust'' cost functions, that employ $\ell_1$ and {\itshape unsquared} $\ell_2$ norms.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> practicalUse.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Sensor failure detection and mitigation}

\subsection{Outliers identification via convex relaxation}
\label{sec:OutIdentif}
The solution can also be used in order to detect sensor failure through outliers identification. In fact, based on the values of the residuals $\restr$ and $\resrot$ obtained by solving the {\itshape 1-} and {\itshape 2-stage} approaches, we will see that it is possible to efficiently classify measurements {\itshape a posteriori} as ``bad'' or correct. Intuitively, if the technique is robust towards the presence of outliers, the residual error over the ``bad'' measurements will be much larger. Therefore, any measurement $k=1, \dots, m$ that has at least one of its corresponding residuals $x_k$ and $y_k$ larger than some suitably fixed thresholds, respectively $\eta^T$ and $\eta^R$, then it is an outlier. A reasonable choice for the thresholds $\eta^T$ and $\eta^R$ is a $2\sigma$ confidence interval. % più su Sensor failure detection che su refinement
%\begin{figure}[H]
%\begin{framed}
%\textbf{input:} translation residuals $\restr$, rotation residuals $\resrot$ \\
%\textbf{output:} outliers indicator vector $\M{\hat \delta}$
%
%\begin{enumerate}
%\item Solve the PGO problem and get residuals $\restr$ and $\resrot$;\\
%\end{enumerate}
%\vspace{-5mm}\textbf{for} $k = 1, \dots, m$
%
%\vspace{1mm}\quad\:\:\:\:\textbf{if} $x_k \geq \eta^T$ \textbf{or} $y_k \geq \eta^R$
%\begin{changemargin}{5mm}{0mm} 
%\begin{enumerate}
%\setcounter{enumi}{1}
%\item set ${\hat \delta}_k = 1$ $\Longrightarrow$ measurement $k$ is outlier
%\end{enumerate}
%
%\:\:\:\:\vspace{-2mm}\textbf{else} 
%
%\begin{enumerate}
%\setcounter{enumi}{2}
%\item set ${\hat \delta}_k = 0$ $\Longrightarrow$ measurement $k$ is not outlier
%\end{enumerate}
%
%\:\:\:\:\vspace{-3mm}\textbf{end} 
%
%\hspace{-5mm}\vspace{0mm}\textbf{end} 
%\end{changemargin} 
%\end{framed}
%\caption{Rounding technique to obtain feasible rotation matrices $\{{\hat R}_i\}_{i=1}^n$ from the solution of the SDP relaxation of the rotation-only problem.}
%\end{figure}




\subsection{Estimate improvement through error mitigation}
\label{sec:ErrorMitigation}
A further possibility we explored is the use outliers detection to perform \cred{some sort of a} refinement step after the procedure described in the previous section, consisting in the resolution of a re-weighted version of the SDP in which the new weights, ${\hat \omega}_k^T$ and ${\hat \omega}_k^R$, associated to each measurement in order to reduce the influence of outlying measurements on the solution. Hence we compute the refined solution ${\hat \MX}$ and the corresponding residuals ${\hat \restr}$ and ${\hat \resrot}$ by minimizing the cost function

\begin{align}
\label{eq:rewProb}
f({\hat \restr}, {\hat \resrot}) =  \sum_{k=1}^m {\hat \omega}_k^T  {\hat x}_k +  {\hat \omega}_k^R  {\hat y}_k
%\quad \text{s. to:}&\quad \|[\mathbf{X}]^{Rt}_{ij} -[\mathbf{X}]^{Rt}_{ii} - \Delta_{ij}\|_1 \leq {\hat x}_k,\quad k=1,\dots,m \nonumber\\
%& \quad \|[\mathbf{X}]^{RR}_{ij} -\bar{ R}_{ij}\|_1 \leq {\hat y}_k,\quad k=1,\dots,m \nonumber\\
%&\quad [\mathbf{X}]^{RR}_{ii}=I_2,\quad i=1,\dots,n \nonumber\\
%& \quad \mathbf{X} \succeq 0  \nonumber
\end{align}

where
\begin{align}
\label{eq:newWeights}
{\hat \omega}_k^T = \frac{1}{\max\{\eta^T,\: x_k\}} \quad \text{and} \quad {\hat \omega}_k^R = \frac{1}{\max\{\eta^R,\: y_k\}}
\end{align}

Again, a suitable choice of the thresholds $\eta^T$ and $\eta^R$ could be respectively $2\sigma_T$ and $2\sigma_R$.




==> preamble_packages.tex <==
%!TEX root = main.tex

% LC: debug
%==========================================================================
%\usepackage{refcheck}
%\usepackage[notref]{showkeys}
%==========================================================================

% LC: to be used for TRO
%==========================================================================
% \usepackage{mathptmx} % assumes new font selection scheme installed
%\usepackage{times} % assumes new font selection scheme installed
%==========================================================================
\usepackage{comment}
\usepackage{siunitx}
\usepackage{relsize}
\usepackage{ifthen}

\usepackage[caption=false]{subfig}

% \begin{comment}
% % Fancy formatting 
% \usepackage[tracking=false,kerning=true,spacing=true]{microtype}
% \usepackage[caption=false]{subfig}

% \usepackage[style=numeric-comp,sorting=none,firstinits=true, maxnames=3,bibstyle=numeric,abbreviate=false,defernums=true,eprint=false,backend=bibtex]{biblatex}
% \renewcommand{\bibfont}{\footnotesize}
% % \DeclareFieldFormat[article]{pages}{#1}%
% % \DeclareFieldFormat[inproceedings]{pages}{#1}%

% \AtEveryBibitem{%
%   \ifentrytype{article}{%
%     \clearfield{pages}%
%   }{%
%   }%
%   \ifentrytype{inproceedings}{%
%     \clearfield{pages}%
%   }{%
%   }%
% }
% \end{comment}

% \bibliography{commons/bib/strings_long}
% \bibliography{commons/bib/all_only_one_w_pages}
% \bibliography{../../references/references}

% \usepackage[noadjust]{cite}
\usepackage[vlined,ruled,linesnumbered]{algorithm2e}
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{rotating}
\usepackage{color}
\usepackage{enumerate}
\usepackage[T1]{fontenc}
\usepackage{psfrag}
\usepackage{epsfig} % for postscript graphics files
%\usepackage{subfigure}
% \usepackage{hyperref}
\usepackage{booktabs}
\usepackage{graphicx,url}
\usepackage{multirow}
\usepackage{array}
\usepackage{latexsym}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{amsthm}
\usepackage{xstring}
\usepackage[noend]{algorithmic}
\usepackage{multirow}
\usepackage{xcolor}
\usepackage{prettyref}
\usepackage{flexisym}
\usepackage{bigdelim}
\usepackage{breqn} % load this last
\usepackage{listings}
\let\labelindent\relax
\usepackage{enumitem}
\usepackage{xspace}
\usepackage{bm}
\graphicspath{{./figures/}}
\usepackage{tikz}
\usetikzlibrary{matrix,calc}


%\usepackage{ifpdf}
% Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% compilation based on whether the output is pdf or dvi.
% usage:
% \ifpdf
%   % pdf code
% \else
%    dvi code
% \fi
% The latest version of ifpdf.sty can be obtained from:
% http://www.ctan.org/tex-archive/macros/latex/contrib/oberdiek/
% Also, note that IEEEtran.cls V1.7 and later provides a builtin
% \ifCLASSINFOpdf conditional that works the same way.
% When switching from latex to pdflatex and vice-versa, the compiler may
% have to be run twice to clear warning/error messages.

% *** GRAPHICS RELATED PACKAGES ***
%
%\ifCLASSINFOpdf
  % \usepackage[pdftex]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../pdf/}{../jpeg/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
%\else
  % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
  % will default to the driver specified in the system graphics.cfg if no
  % driver is specified.
  % \usepackage[dvips]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../eps/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.eps}
%\fi


\usepackage{mdwlist}
\let\stditemize\itemize
\let\endstditemize\enditemize
\let\itemize\undefined
\makecompactlist{itemize}{stditemize}

%\let\stdenumerate\enumerate
%\let\endstdenumerate\endenumerate
%\let\enumerate\undefined
%\makecompactlist{enumerate}{stdenumerate}
 


==> resultsIncreasingN.tex <==
For increasing number of poses $n$, the robustness is not lost. In fact, as shown in Fig.~\ref{fig:aveDistFromGTn}, the mean error over node's orientation and position decreases for increasing $n$. While Fig.~\ref{fig:aveDistFromGTn} considers $\ell_2$ {\itshape 2-stage} approach, 
similar conclusions hold for the other 2-stage approaches.
% The proposed approach is thus scalable and its effectiveness  improves for larger pose graphs. \cblue{Although, as already mentioned above, the general purpose SDP solver used in our current implementation scales poorly in the problem size (it requires \cred{more than $1$min to solve an instance with $50$ poses}). This motivates the employment of IRLS to tackle the {\itshape 2-stage} approaches as explained in Subsection~\ref{sec:FastNumericalSolver}.}



\begin{figure}[h]
\begin{minipage}{\columnwidth}
\begin{tabular}{cc}
\hspace{-5mm}
\begin{minipage}{0.5\columnwidth}%
\includegraphics[scale=0.235]{figures/comparAveTran_n} 
\vspace{-5mm} \\ 
\centering (a) 
\end{minipage}%
&
\hspace{-5mm}
\begin{minipage}{0.5\columnwidth}%
\centering
%\vspace{-3.5mm}
\includegraphics[scale=0.235]{figures/comparAveRot_n} 
\vspace{-5mm} \\ 
\centering (b) 
\end{minipage}%  
\end{tabular} 
\end{minipage}%
\caption{Mean error (in Log scale) over (a) translations and (b) rotations obtained using the $\ell_2$ 
{\itshape 2-stage} approach for increasing number of nodes and different values of $p^{out}$. 
%$\sigma_R = 0.01$, $\sigma_T = 0.1$ and $p=0.5$.
\label{fig:aveDistFromGTn}}
\vspace{-0.5cm}
\end{figure}

==> rotationRoundingAlgorithm.tex <==
%!TEX root = Special Issue COMPENG2016 - Draft.tex

%\vspace*{-\baselineskip}
\begin{algorithm}[h!]
\SetAlgoLined
\textbf{Input:} \ $\hatMX$\; 
\textbf{Output:} \ rotation estimates $\hatMR_i$, $i=1,\ldots,n$ \; 
\indent $\hatMZ \leftarrow$ compute rank-2 approximation of $\hatMX$, via SVD \;
 \For{$i = 1,\ldots,n$}{
  compute SVD of the $i$-th $2 \times 2$ block of $\hatMZ$: \\
  $\hatMZ_i = \MU_i \MSigma_i \MV_i\tran$ \label{eq:rank2approx} \\
  \cblue{project to \SOtwo: $\hatMR_i = \MU_i \MJ_i \MV_i\tran $, where $ \MJ_i= {\tiny \matTwo{ 1 & 0 \\ 0 & \text{det}(\MU_i \MV_i\tran)}}$}
  \label{eq:projectSO2}
 }
 \textbf{return} $\hatMR_i$, $i=1,\ldots,n$.
 \caption{Rotation Rounding. \label{alg:rotRound}}
\end{algorithm}
%\vspace*{-\baselineskip} 

% \vspace{-1mm} 
% \begin{figure}[H]
% \begin{framed}
% \textbf{input:} estimated Gram matrix $\mathbf{\hat G}$ \\
% \textbf{output:} estimated rotation matrices $\{{\hat R}_i\}_{i=1}^n$
% \begin{enumerate}
% \item Compute matrix $Q = [q_1 \:\: q_2] \in \Real{2n\times2}$, whose columns are the eigenvectors corresponding to the $2$ largest eigenvalues of $\mathbf{\hat G}$;\\
% \end{enumerate}
% \vspace{-4mm}\textbf{for} $i = 1, \dots, n$
% \begin{changemargin}{5mm}{0mm} 
% \begin{enumerate}
% \setcounter{enumi}{1}
% \item perform singular value decomposition of each of the $n$ submatrices of $Q = [Q_1\tran  \dots Q_n\tran ]\tran $ of size $2\times2$
% \begin{align}
% Q_i = U_i\Sigma_iV_i\tran ; \nonumber
% \end{align}
% \item ${\hat R}_i = U_i \mathbf{J}_i V_i\tran $, where $ \mathbf{J}_i= \left[ \begin{array}{cc} 1 & 0 \\ 0 & \text{det}(U_iV_i\tran ) \end{array} \right]$.
% \end{enumerate}
% \end{changemargin} 
% \end{framed}
% %\caption{Rounding technique to obtain feasible rotation matrices $\{{\hat R}_i\}_{i=1}^n$ from the solution of the SDP relaxation of the rotation-only problem.}
% \end{figure}
